BIASINSPECTOR: Detecting Bias in Structured Data through LLM Agents

Detecting biases in structured data is a complex and time-consuming task. Existing automated techniques are limited in diversity of data types and heavily reliant on human case-by-case handling, resulting in a lack of generalizability. Currently, large language model (LLM)-based agents have made significant progress in data science, but their ability to detect data biases is still insufficiently explored. To address this gap, we introduce the first end-to-end, multi-agent synergy framework, BIASINSPECTOR, designed for automatic bias detection in structured data based on specific user requirements. It first develops a multi-stage plan to analyze user-specified bias detection tasks and then implements it with a diverse and well-suited set of tools. It delivers detailed results that include explanations and visualizations. To address the lack of a standardized framework for evaluating the capability of LLM agents to detect biases in data, we further propose a comprehensive benchmark that includes multiple evaluation metrics and a large set of test cases. Extensive experiments demonstrate that our framework achieves exceptional overall performance in structured data bias detection, setting a new milestone for fairer data applications.

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables_.tex <==
\begin{table}[H]
\centering
\caption{Sample questions from the constructed taskset (excerpt).}
\label{tab:taskset-samples}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|p{4.5cm}|c|p{2cm}|p{3.5cm}|}
\hline
\textbf{Question} & \textbf{Type} & \textbf{Feature(s)} & \textbf{Bias Significance} \\
\hline
Can you check if the age distribution across individuals is balanced, or do certain age groups dominate? & Distribution & age (Numerical) & Imbalanced age groups may skew income-related insights. \\
\hline
How does the distribution of work class look to you? Are there any work classes that appear to be overrepresented? & Distribution & workclass (Categorical) & Uneven representation can bias analysis of income across sectors. \\
\hline
From your perspective, is the distribution of education levels spread fairly, or do certain levels dominate? & Distribution & education (Categorical) & Dominance in education levels may affect fairness in outcome evaluation. \\
\hline
In your view, how does the marital status distribution appear? Are any marital statuses overrepresented? & Distribution & marital-status (Categorical) & Skewed marital status can distort socio-economic impact assessments. \\
\hline
Do certain occupations dominate the dataset, or is the distribution of occupations relatively even? & Distribution & occupation (Categorical) & Occupation imbalance may lead to biased interpretation of income disparities. \\
\hline
\end{tabular}
\end{table}


==> tools_info_in_evaluation_agent.tex <==
\begin{longtable}{|p{5cm}|p{8cm}|}
\caption{Description of tools in the evaluation agent toolset.}\label{tab:evaluation-tools} \\
\hline
\multicolumn{2}{|c|}{\rule{0pt}{3ex}\textbf{Automated Agent Evaluation Tools}\rule{0pt}{3ex}} \\
\hline
\textbf{Tool} & \textbf{Description} \\
\hline
\endfirsthead

\multicolumn{2}{c}{\textit{(Continued from previous page)}} \\
\hline
\textbf{Tool} & \textbf{Description} \\
\hline
\endhead

\hline \multicolumn{2}{|r|}{\textit{Continued on next page}} \\
\hline
\endfoot

\hline
\endlastfoot

get\_user\_input\_tool & Captures user input dynamically during an interaction and formats it as a dictionary to be added to the agent's conversation. \\
\hline
read\_json\_log & Reads a JSON formatted log file, extracting and organizing log entries. \\
\hline
read\_markdown\_log & Reads a Markdown formatted log file, extracting headers, bold text, and regular text as structured log entries. \\
\hline
read\_bias\_report\_pdf & Reads a bias detection report in PDF format, extracting both textual and graphical information. \\
\hline
generate\_evaluation\_report\_pdf & Generates a flexible evaluation report in PDF format, combining text narratives and visual charts as specified in the input. \\
\hline
\end{longtable}


==> tools_info_in_toolset.tex <==
\begin{longtable}{|p{5cm}|p{8cm}|}
\caption{Description of tools in toolset.} \\
\hline
\multicolumn{2}{|c|}{\rule{0pt}{3ex}\textbf{Data Loading and Preprocessing Tools}\rule{0pt}{3ex}} \\
\hline
\textbf{Tool} & \textbf{Description} \\
\hline
\endfirsthead
\multicolumn{2}{c}{\textit{(Continued from previous page)}} \\
\hline
\textbf{Tool} & \textbf{Description} \\
\hline
\endhead
\hline \multicolumn{2}{|r|}{\textit{Continued on next page}} \\
\hline
\endfoot
\hline
\endlastfoot
get\_csv\_features & Reads a CSV file and returns all feature names (column names) \\
\hline
load\_csv\_file & Loads a CSV file and returns it as a Pandas DataFrame \\
\hline
extract\_single\_column & Extracts a single column from a CSV file and saves it as a new dataset \\
\hline
extract\_two\_columns & Extracts two columns from a CSV file and saves them as a new dataset \\
\hline
clean\_missing\_values & Cleans missing or invalid values from specified columns and saves the cleaned dataset \\
\hline
normalize\_or\_standardize\_data & Applies 'normalize' or 'standardize' to a specified column and saves the result as a new dataset \\
\hline
group\_and\_aggregate & Groups the data by a specified column and applies an aggregation function on another column \\
\hline
\multicolumn{2}{|c|}{\rule{0pt}{3ex}\textbf{Detect and Analysis Tools}\rule{0pt}{3ex}} \\
\hline
\textbf{Tool} & \textbf{Description} \\
\hline
categorical\_distribution\_shannon \_balance & Analyzes the distribution bias of a categorical column using Shannon entropy and Balance metric \\
\hline
categorical\_distribution\_shannon \_balance & Analyzes the distribution bias of a categorical column using Shannon entropy and Balance metric. \\
\hline
categorical\_distribution\_max \_min\_ratio & Analyzes the distribution bias of a categorical column using the max/min ratio of categories. \\
\hline
categorical\_distribution\_entropy & Analyzes the distribution bias of a categorical column using Shannon entropy and normalized entropy. \\
\hline
categorical\_distribution\_gini & Analyzes the distribution bias of a categorical column using the Gini Index with Laplace smoothing and sample size correction. \\
\hline
categorical\_distribution\_relative \_risk & Analyzes the distribution bias of a categorical column using relative risk by comparing observed and expected frequencies. \\
\hline
numerical\_distribution\_skewness & Analyzes the distribution bias of a numerical column using skewness to assess asymmetry in the data. \\
\hline
numerical\_distribution\_kurtosis & Analyzes the distribution bias of a numerical column using kurtosis to assess the "tailedness" of the distribution. \\
\hline
numerical\_distribution\_outlier & Analyzes the distribution bias of a numerical column using Z-score outlier detection to assess the percentage of outliers. \\
\hline
numerical\_distribution\_cohens \_d\_mad & Analyzes the distribution bias of a numerical column using Cohen's d, calculated with Median Absolute Deviation (MAD) for robustness against outliers. \\
\hline
numerical\_distribution\_quantile \_deviation & Analyzes the distribution bias of a numerical column using quantile deviation, calculated as the ratio of Q3-Q2 to the interquartile range (IQR). \\
\hline
categorical\_categorical \_correlation\_cramers\_v & Analyzes the correlation bias between two categorical columns using Cramér's V, which measures association strength based on the chi-square statistic. \\
\hline
categorical\_categorical \_correlation\_elift & Analyzes the correlation bias between two categorical columns using Elift, calculated as the ratio of confidence(X -> Y) to confidence(Y). \\
\hline
categorical\_categorical \_correlation\_statistical\_parity & Analyzes the correlation bias between two categorical columns using statistical parity and Z-scores to assess differences in proportions between groups. \\
\hline
categorical\_categorical \_correlation\_lipschitz & Analyzes the correlation bias between two categorical columns using a Lipschitz function to measure distribution loss differences between groups. \\
\hline
categorical\_categorical \_correlation\_total\_variation & Analyzes the correlation bias between two categorical columns using Total Variation Distance (TVD) to measure the difference between group-specific and overall distributions. \\
\hline
categorical\_numerical\_correlation \_max\_abs\_mean & Analyzes the correlation bias between a categorical and a numerical column by computing the standardized mean for each category and evaluating the maximum absolute mean (N value). \\
\hline
categorical\_numerical\_correlation \_cohens\_d & Analyzes the correlation bias between a categorical and a numerical column using Cohen's d to measure the effect size based on an independent t-test. \\
\hline
categorical\_numerical\_correlation \_standardized\_difference & Analyzes the correlation bias between a categorical and a numerical column using Standardized Difference (SD), calculated with mean and Median Absolute Deviation (MAD). \\
\hline
categorical\_numerical\_correlatio n\_causal\_effect & Analyzes the correlation bias between a categorical treatment and a numerical outcome using causal inference to estimate the Average Causal Effect (ACE). \\
\hline
categorical\_numerical\_correlation \_pse & Analyzes the correlation bias between a categorical and a numerical column using Path-Specific Effect (PSE), along with the Average Direct Effect (ADE) and Average Indirect Effect (AIE). \\
\hline
numerical\_numerical\_correlation \_pearson & Analyzes the correlation bias between two numerical columns using Pearson correlation to measure the strength of their linear relationship. \\
\hline
numerical\_numerical\_correlation \_nmi & Analyzes the correlation bias between two numerical columns using Normalized Mutual Information (NMI) after discretizing the data into bins. \\
\hline
numerical\_numerical\_correlation \_hgr\_approximation & Analyzes the correlation bias between two numerical columns using HGR approximation and chi-squared 
 divergence, combining Pearson correlation and Kernel Density Estimation (KDE) to assess the strength of the relationship. \\

\hline
numerical\_numerical\_correlation \_wasserstein & Analyzes the correlation bias between two numerical columns using Wasserstein-2 distance to measure the differences between their distributions. \\
\hline
numerical\_numerical\_correlation \_hsic & Analyzes the correlation bias between two numerical columns using the Hilbert-Schmidt Independence Criterion (HSIC) with Radial Basis Function (RBF) kernels to measure their dependence. \\
\hline
\multicolumn{2}{|c|}{\rule{0pt}{3ex}\textbf{Visualization Tools}\rule{0pt}{3ex}} \\
\hline
\textbf{Tool} & \textbf{Description} \\
\hline
plot\_bar\_chart & Generates a bar chart for a specified column in a CSV file and saves it as an image. \\
\hline
plot\_pie\_chart & Generates a pie chart for a specified column in a CSV file and saves it as an image. \\
\hline
plot\_horizontal\_bar\_chart & Generates a horizontal bar chart for a specified column in a CSV file and saves it as an image. \\
\hline
plot\_treemap & Generates a treemap for a specified column in a CSV file and saves it as an image. \\
\hline
plot\_heatmap & Generates a heatmap for the frequency distribution of a specified column in a CSV file and saves it as an image. \\
\hline
plot\_correlation\_heatmap & Generates a correlation heatmap for multiple specified columns in a CSV file and saves it as an image. \\
\hline
plot\_stacked\_bar\_chart & Generates a stacked bar chart for two specified categorical columns in a CSV file and saves it as an image. \\
\hline
plot\_grouped\_bar\_chart & Generates a grouped bar chart for two specified categorical columns in a CSV file and saves it as an image. \\
\hline
plot\_box\_plot & Generates a box plot for a categorical column and a numeric column in a CSV file and saves it as an image. \\
\hline
\multicolumn{2}{|c|}{\rule{0pt}{3ex}\textbf{Miscellaneous Tools}\rule{0pt}{3ex}} \\
\hline
\textbf{Tool} & \textbf{Description} \\
\hline
get\_user\_input\_tool & Captures user input dynamically during an interaction and formats it as a dictionary to be added to the Agent's conversation. \\
\hline
get\_all\_reference\_intentions & Retrieves all intentions from the references JSON file, including each reference's id and corresponding intention. \\
\hline
get\_reference\_method\_by\_id & Retrieves the method for a specific reference by ID from the references JSON file. \\
\hline
generate\_bias\_report\_pdf & Generates a bias detection report in PDF format, combining text and charts as specified in the input. \\
\hline
execute\_python\_code & Executes the provided Python code and returns the printed output, if any. 

\label{tab:tools_info_in_toolset}
\end{longtable}

